The Impact of Negation on the Complexity of the Shapley Value in Conjunctive Queries

The Shapley value is a conventional and well-studied function for determining the contribution of a player to the coalition in a cooperative game. Among its applications in a plethora of domains, it has recently been proposed to use the Shapley value for quantifying the contribution of a tuple to the result of a database query. In particular, we have a thorough understanding of the tractability frontier for the class of Conjunctive Queries (CQs) and aggregate functions over CQs. It has also been established that a tractable (randomized) multiplicative approximation exists for every union of CQs. Nevertheless, all of these results are based on the monotonicity of CQs. In this work, we investigate the implication of negation on the complexity of Shapley computation, in both the exact and approximate senses. We generalize a known dichotomy to account for negated atoms. We also show that negation fundamentally changes the complexity of approximation. We do so by drawing a connection to the problem of deciding whether a tuple is "relevant" to a query, and by analyzing its complexity.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

==> self-joins.tex <==
%\subsection{BCQs with self-joins}
The proof of Theorem~\ref{thm:sjfbcq} heavily relies on the assumption that the query is self-join free. In the remainder of this section, we provide an insight into the complexity of the problem for queries with self-joins. As Livshits et al.~\cite{DBLP:journals/corr/abs-1904-08679} only considered self-join free queries, our result here is the first complexity result on the computation of the Shapley value for queries with self-joins.

We consider queries in $\BCQneg$ that are \e{polarity-consistent}; hence, we first formally define such queries.

\begin{definition}[Polarity Consistency]
A relation $R$ is \e{polarity-consistent} w.r.t.~a CQ $q$ if it occurs only in positive atoms or only in negative atoms of $q$. A CQ $q$ is polarity-consistent if every relation occurring in $q$ is polarity-consistent.
\end{definition}

As an example, the query $q_3$ of our running example (defined in Example~\ref{example:queries}) is polarity-consistent, while the query $q_4$ is not, since the relations \rel{TA} and \rel{Reg} occur both as a positive and as a negative atom in the query. The class of polarity-consistent queries will play an important role in our analysis of the approximate computation of the Shapley value in Section~\ref{sec:approx}. We prove the following.

%For simplicity, we assume that each edge in $\graph(q)$ is annotated by the corresponding atom connecting the two variables. We refer to the aforementioned path between $x$ and $y$ in $\graph(q)$ as a \e{non-hierarchical variable path} in $q$, and we refer to the path of atoms $\beta_1-\dots-\beta_m$ along the edges of this variable path as a \e{non-hierarchical atom path}. Note that two variables can occur together in various different atoms of $q$; hence, each variable path may be associated with multiple atom paths. We will now prove that computing $\shp(D,q,f)$ is $\FP$-complete for a subclass of $\nhpath$ that contains every query in $\nhpath$ that has a non-hierarchical atom path in which the first and last atoms are unique (i.e., appear only once in $q$).

%We first recall the definition of minimal BCQs~\cite{DBLP:books/aw/AbiteboulHV95}. We say that a BCQ $q$ is \e{minimal} if there is no BCQ $q'$ such that $|q'|<|q|$ (where $|q|$ is the number of atoms of $q$), and $D\models q$ if and only if $D\models q'$ (i.e., $q$ and $q'$ are equivalent). A query $q$ is \e{satisfiable} if there exists a database $D$ such that $D\models q$. Note that satisfiability can be checked in polynomial time for queries in $\BCQneg$~\cite{DBLP:conf/icdt/WeiL03}. Clearly, if a query $q$ is not satisfiable, then $\shp(D,q,f)=0$ for every database $D$ and fact $f$. Hence, our hardness result applies only to satisfiable queries.
%We prove the following. 

%we show that the exact Shapley value for non-hierarchical queries is hard for the class of safe $BCQ$ even with self-joins when the minimized query is satisfiable.


\def\thmbcqsj{
Let $q\in\BCQneg$ be a polarity-consistent query containing a non-hierarchical triplet $(\alpha_x,\alpha_{x,y},\alpha_y)$ where the relation $R^{\alpha_{x,y}}$ occurs only once in the query. Then, computing $\shp(D,q,f)$ is $\FP$-complete.
}
\begin{theorem} \label{thm:bcqn_sj}
\thmbcqsj
\end{theorem}

To prove the theorem, we construct a reduction from the problem of computing $\shp(D,q',f)$ where $q'$ is one of $\cqrst$, $\cqrnst$, $\cqnrsnt$ or $\cqrsnt$ (depending on the polarity of the atoms $\alpha_x$, $\alpha_y$, and $\alpha_{x,y}$) under the following assumptions: \e{(1)} all the facts of $S$ are exogenous, and \e{(2)} for every fact $S(\val{a},\val{1})$ in $D$, both facts $R(\val{a})$ and $T(\val{1})$ are in $D$. The instances constructed in the proofs of hardness for all three queries satisfy these conditions; hence, the problems remain hard under these assumptions. The idea is very similar to the proof of Lemma~\ref{lemma:sjfbcq_hard}. We also assume for simplicity that the set of values used in the facts of $R^D$ and the set of values used in the facts of $T^D$ are disjoint.

The idea is the following. We use the atoms $\alpha_x$ and $\alpha_y$ to represent the atoms $R(x)$ and $T(y)$ in $q'$, and we use the atom $\alpha_{x,y}$ to represent the connections between them (i.e., the atom $S(x,y)$). We use the assumption that the relation corresponding to the atom $\alpha_{x,y}$ occurs only once in the query to ensure that we do not create new connections between pairs of values of $x$ and $y$. If $\alpha_x$ and $\alpha_y$ are both positive, the reduction is from the problem of computing $\shp(D,\cqrst,f)$, if both atoms are negative, the reduction is from computing $\shp(D,\cqnrsnt,f)$, and if one atom is positive while the other is negative, the reduction is from computing $\shp(D,\cqrsnt,f)$.

Formally, given an input database $D$ to the first problem, we build a database $D'$ in the following way. For every fact $f=R(\val{a})$ we assign the value $\val{a}$ to the variable $x$ in $\alpha_x$ and the value $\odot$ to the rest of the variables, and we add the corresponding fact $f'$ to the relation $R^{\alpha_x}$ in $D'$. The fact $f'$ will be endogenous if and only if $f$ is endogenous. Similarly, for every fact $f=T(\val{1})$ we assign the value $\val{1}$ to the variable $y$ in $\alpha_y$ and the value $\odot$ to the rest of the variables, and we add the corresponding fact $f'$ to the relation $R^{\alpha_y}$ in $D'$. Again, the fact $f'$ will be endogenous if and only if $f$ is endogenous.
Next, for every fact $S(\val{a},\val{1})$ in $D$ and an atom $\alpha$ in $q$ that is not one of $\alpha_x$ or $\alpha_y$, we assign the value $\val{a}$ to the variable $x$, the value $\val{1}$ to the variable $y$, and the value $\odot$ to the rest of the variables, and we add the corresponding fact to the relation $R^\alpha$ in $D'$ if we have not added this fact to $D'$ already. Every such fact will be exogenous. Note that we have that $|D\endo|=|D\endo'|$.

Now, given the database $D'$ we construct a database $D''$ which will be the input to our problem in the following way. First, we define the domain of every variable in $q$. The domain of $x$ will consist of the values occurring in the relation $R$ in $D$, the domain of $y$ will consist of the values occurring in the relation $T$ in $D$, and the domain of the rest of the variables will consist of a single value $\odot$. We first copy all the endogenous facts from $D'$ to $D''$. Then, for every relation $R$ in $D'$ corresponding to positive atoms of $q$ (recall that $q$ is polarity-consistent), we copy every exogenous fact from $R^{D'}$ to $R^{D''}$. For every relation $R\neq R^{\alpha_{x,y}}$ in $D'$ corresponding to negative atoms of $q$, we add to $R^{D''}$ every exogenous fact over the aforementioned domain if and only if it does not occur in $R^{D'}$. That is, for every atom $\alpha$ (that is not one of $\alpha_x$, $\alpha_y$ or $\alpha_{x,y}$) in $q$ over the relation $R$, we consider every possible mapping of the variables in $\alpha$ to their domains, and add the corresponding exogenous fact to $R^{D''}$ if and only if it does not appear as an exogenous fact in $R^{D'}$. Finally, if $\alpha_{x,y}$ is negative, we add to $R^{\alpha_{x,y}}$ in $D''$ every fact $f$ obtained from a mapping of the variables in $\alpha_{x,y}$ to values from the whole domain (i.e., we do not restrict the domain of each variable) if and only if $f$ does not appear in $R^{\alpha_{x,y}}$ in $D'$. Note that since we did not change the endogenous facts, we have that $|D\endo|=|D'\endo|=|D''\endo|$.

We will now prove that for every endogenous fact $f_1$ in $D$ and its corresponding fact $f_2$ in $D''$ (i.e., the fact that was generated from $f_1$) it holds that $\shp(D,q',f_1)=\shp(D'',q,f_2)$ (recall that $q'$ is one of $\cqrst$, $\cqnrsnt$, $\cqrsnt$). We start by proving the following. 

\begin{lemma}\label{yes_to_yes}
Let $E\subseteq D\endo$ and let $E''$ be the set of corresponding facts in $D''\endo$. If $(D\exo\cup E)\models q'$ then $(D''\exo\cup E'')\models q$.
\end{lemma}
\begin{proof}
Since $(D\exo\cup E)\models q'$ there is a mapping $h$ from the variables of $q'$ to the domain of $D$ where $h(x)=\val{a}$ for some value $\val{a}$ from the domain of $R^D$ and $h(y)=\val{1}$ for some value $\val{1}$ from the domain of $T^D$ such that $h$ maps every positive atom and none of the negative atoms of $q'$ to a fact of $D\exo\cup E$. We claim that the mapping $h'$ such that $h'(x)=h(x)$, $h'(y)=h(y)$, and $h'(w)=\odot$ for the rest of the variables, maps every positive atom and none of the negative atoms of $q$ to facts of $D''\exo\cup E''$; hence $(D''\exo\cup E'')\models q$.

When considering the fact $S(\val{a},\val{1})$ in the construction of $D'$, we have created a mapping $h'$ from the variables of $q$ such that $h'(x)=\val{a}$, $h'(y)=\val{1}$, and $h'(w)=\odot$ for the rest of the variables, and we have added all the resulting facts (associated with atoms that are not one of $\alpha_x$ or $\alpha_y$) to $D'$ (as exogenous facts). When constructing $D''$ we have removed every such fact if it was generated from a negative atom of $q$. Hence, $h'$ is a mapping from the variables of $q_{\setminus\set{\alpha_x,\alpha_y}}$ (which is the query obtained from $q$ by removing the atoms $\alpha_x$ and $\alpha_y$) to the domain of $D''$ such that every positive atom and none of the negative atoms of $q$ appears as a fact in $D\exo''$. Moreover, it holds that $R(\val{a})\in D\endo$ if and only $h'(\alpha_x)\in D''\endo$ and similarly $T(\val{1})\in D\endo$ if and only if $h'(\alpha_y)\in D''\endo$.

It is only left to show that there is no negative atom of $q$ that is mapped by $h'$ to a fact in $D''\endo$. Let us assume, by way of contradiction, that a negative atom $\beta$ of $q$ is mapped by $h'$ to a fact $f$ in $D''\endo$, and assume, without loss of generality, that $f$ belongs to the relation $R^{\alpha_x}$ in $D''$. Since $q$ is polarity-consistent, the atom $\alpha_x$ is a negative atom as well. Moreover, in this case, the relation $R$ appears as a negative atom in $q'$. From the construction of $D''$, for every endogenous fact $f$ in the relation $R^{\alpha_x}$ in $D''$ there is a homomorphism from $\alpha_x$ to $f$ that maps the variable $x$ to a value from its domain, the variable $y$ to a value from its domain, and the rest of the variables to $\odot$. If $h'$ maps $\beta$ to $f$, then there is also a homomorphism from $\beta$ to $\alpha_x$ (and from $\alpha_x$ to $\beta$) where $x$ is mapped to itself. We conclude that $h'$ maps the atom $\alpha_x$ to the fact $f$. From the construction of $D''$, we have that $R(\val{a})\in E$, which is a contradiction to the fact that $R$ appears as a negative atom in $q$ and $(D\exo\cup E)\models q$.
\end{proof}

Next, we prove the following.
\begin{lemma}\label{lemma:not_to_not}
Let $E\subseteq D\endo$ and let $E''$ be the set of corresponding facts in $D''\endo$. If $(D\exo\cup E)\not\models q'$ then $(D''\exo\cup E'')\not\models q$.
\end{lemma}
\begin{proof}
Let us assume, by way of contradiction, that $(D''\exo\cup E'')\models q$. Then, there is a mapping $h$ from the variables of $q$ to the domain of $D''$ that maps every positive atom and none of the negative atoms of $q$ to a fact in $D''\exo\cup E''$. In particular, the atom $\alpha_{x,y}$, is mapped to a fact of $D''\exo\cup E'$ if and only if it is positive. From the construction of $D''$ and the uniqueness of the atom (i.e., the fact that its relation does not appear in another atom of $q$), we have that if $\alpha_{x,y}$ is positive, then $h$ maps $\alpha_{x,y}$ to a fact of $D''\exo$ if and only there exists a fact $S(\val{a},\val{1})$ in $D$ such that $h(x)=\val{a}$ and $h(y)=\val{1}$. If $\alpha_{x,y}$ is negative, then $h$ does not map $\alpha_{x,y}$ to a fact of $D''\exo$ if and only if there exists a fact $S(\val{a},\val{1})$ in $D$ such that $h(x)=\val{a}$ and $h(y)=\val{1}$.

We claim that the mapping $h$ is such that every positive atom and none of the negative atoms of $q'$ is mapped to a fact of $D\exo\cup E$, which is a contradiction to the fact that $(D\exo\cup E)\not\models q$. We have already established, that there exists an exogenous fact $S(\val{a},\val{1})$ in $D$ such that $h(x)=\val{a}$ and $h(y)=\val{1}$. It is only left to show that the fact $R(\val{a})$ belongs to $E$ if and only if $R$ occurs as a positive atom in $q'$, and, similarly, the fact $T(\val{1})$ belongs to $E$ if and only if $T$ occurs as a positive atom in $q'$.

If $\alpha_x$ is a positive atom, then there is a fact $f$ in the relation $R^{\alpha_x}$ in $D''$ obtained from $\alpha_x$ by mapping the variable $x$ to the value $\val{a}$ and the rest of the variables to the value $\odot$, such that $f\in E''$. In this case, the relation $R$ also appears in $q'$ as a positive atom and the fact $f'=R(\val{a})$ corresponding to $f$ appears in $E$. If $\alpha_x$ is a negative atom (in which case, the relation $R$ occurs in $q'$ as a negative atom), then the fact $f$ does not appear in $E''$ (or, otherwise, $D''\exo\cup E''$ will not satisfy $q$), which implies that the fact $f'$ does not appear in $E$. We can similarly show that the fact $T(\val{1})$ appears in $E$ if and only if its corresponding fact appears in $E'$, and that concludes our proof.
\end{proof}

The remainder of the proof is rather straightforward based on these two lemmas. Since the total number of permutations of the facts in $D\endo$ and $D''\endo$ is equal, we only need to show that the number of permutations where $f_1$ changes the result of $q'$ is equal to the number of permutations where $f_2$ changes the result of $q$. Let $\sigma=g_1,\dots,g_n$ be a permutation of the endogenous facts in $D$ and let $\sigma'=g_1',\dots,g_n'$ be the corresponding permutation of the endogenous facts in $D''$. We will show that $f_1$ changes the result of $q'$ in $\sigma$ if and only if $f_2$ changes the result of $q$ in $\sigma'$.

If $f_1$ changes the result of $q'$ from false to true in $\sigma$, we have that $(D\exo\cup\sigma_{f_1})\not\models q'$ and $(D\exo\cup\sigma_{f_1}\cup\{f_1\})\models q'$. In this case, Lemma~\ref{lemma:not_to_not} implies that $(D''\exo\cup\sigma_{f_2}')\not\models q$ and Lemma~\ref{yes_to_yes} implies that $(D''\exo\cup\sigma'_{f_2}\cup\{f_2\})\models q$. Hence, $f_2$ changes the result of $q$ from false to true in $\sigma'$. Similarly, if $f_1$ changes the result of $q'$ from true to false in $\sigma$, we have that $(D\exo\cup\sigma_{f_1})\models q'$ and $(D\exo\cup\sigma_{f_1}\cup\{f_1\})\not\models q'$. In this case, Lemma~\ref{yes_to_yes}
implies that $(D''\exo\cup\sigma_{f_2}')\models q$ and Lemma~\ref{lemma:not_to_not} implies that $(D''\exo\cup\sigma'_{f_2}\cup\{f_2\})\not\models q$. Hence, $f_2$ changes the result of $q$ from false to true in $\sigma'$.

Finally, if $f_1$ does not change the result of $q'$ from false to true in $\sigma$, we have that either $(D\exo\cup\sigma_{f_1})\models q'$ or $(D\exo\cup\sigma_{f_1}\cup\{f_1\})\not\models q'$. In the first case, Lemma~\ref{yes_to_yes} implies that $(D''\exo\cup\sigma_{f_2}')\models q$ and in the second case Lemma~\ref{lemma:not_to_not} implies that $(D''\exo\cup\sigma'_{f_2}\cup\{f_2\})\not\models q$. Hence, $f_2$ does not change the result of $q$ from false to true in $\sigma'$. Similarly, if $f_1$ does not change the result of $q'$ from true to false in $\sigma$, we have that either $(D\exo\cup\sigma_{f_1})\not\models q'$ or $(D\exo\cup\sigma_{f_1}\cup\{f_1\})\models q'$. In the first case, Lemma~\ref{lemma:not_to_not}
implies that $(D''\exo\cup\sigma_{f_2}')\not\models q$ and in the second case Lemma~\ref{yes_to_yes} implies that $(D''\exo\cup\sigma'_{f_2}\cup\{f_2\})\models q$. Hence, $f_2$ does not change the result of $q$ from false to true in $\sigma'$.

\begin{example}
Consider the query $q()\dl R(x),S(x,y),R(y)$. Since $q$ is polarity consistent and $S(x,y)$ occurs only once in the query, Theorem~\ref{thm:bcqn_sj} implies that computing $\shp(D,q,f)$ is $\FP$-complete. Next, consider the query $q_2$ of our running example. This query is also polarity consistent, and the atom $\rel{Reg}(x,y)$ is the only atom over the relation $\rel{Reg}$; hence, again, Theorem~\ref{thm:bcqn_sj} implies that computing $\shp(D,q_2,f)$ is $\FP$-complete. On the other hand, the query $q()\dl R(x),S(x,y),\neg R(y)$ is not sign-consistent and Theorem~\ref{thm:bcqn_sj} cannot be used to classify the complexity of this query; however, we can prove that computing $\shp(D,q,f)$ is $\FP$-complete using a simple reduction from the problem of computing $\shp(D,\cqrsnt,f)$.
\end{example}



